Fed-TGAN: Federated Learning Framework for Synthesizing Tabular Data

Generative Adversarial Networks (GANs) are typically trained to synthesize data, from images and more recently tabular data, under the assumption of directly accessible training data. Recently, federated learning (FL) is an emerging paradigm that features decentralized learning on client's local data with a privacy-preserving capability. And, while learning GANs to synthesize images on FL systems has just been demonstrated, it is unknown if GANs for tabular data can be learned from decentralized data sources. Moreover, it remains unclear which distributed architecture suits them best. Different from image GANs, state-of-the-art tabular GANs require prior knowledge on the data distribution of each (discrete and continuous) column to agree on a common encoding -- risking privacy guarantees. In this paper, we propose Fed-TGAN, the first Federated learning framework for Tabular GANs. To effectively learn a complex tabular GAN on non-identical participants, Fed-TGAN designs two novel features: (i) a privacy-preserving multi-source feature encoding for model initialization; and (ii) table similarity aware weighting strategies to aggregate local models for countering data skew. We extensively evaluate the proposed Fed-TGAN against variants of decentralized learning architectures on four widely used datasets. Results show that Fed-TGAN accelerates training time per epoch up to 200% compared to the alternative architectures, for both IID and Non-IID data. Overall, Fed-TGAN not only stabilizes the training loss, but also achieves better similarity between generated and original data. Our code is released at https://github.com/zhao-zilong/Fed-TGAN.

==> temp.tex <==
This experiments uses one server and five clients. Each client is provided with a copy of the full real dataset. This represents the ideal case with perfectly identical clients, i.e. each client has iid data. We compare in particular \algo, \mdtgan and \central. Since in this case the aggregation weights of \algo are the same as for \vanilla  due to the identical data, we skip \vanilla. Results for the Intrusion dataset are shown in Fig.~\ref{fig:5full_intrusion}. Avg-JSD and Avg-WD are presented by both epoch and time (in seconds) as different architectures spend vastly different time per epoch. For categorical columns \algo converges faster both by epoch and by time (see Fig.\ref{fig:5full_intrusionjsd} and \ref{fig:5full_intrusionjsdt}). Moreover, the Avg-JSD of \mdtgan converges quite slowly after epoch 28. For continuous columns, from the perspective of number of epochs, Avg-WD for \algo converges faster at the beginning, then becomes slightly worse than the Avg-WD for \mdtgan (see Fig.\ref{fig:5full_intrusionwd}. However, inspecting the result by time, \algo not only converges faster, but also achieves a lower Avg-WD than the other two architectures (see Fig.\ref{fig:5full_intrusionwdt}. The performance gap between the centralized approach and \algo may look counter-intuitive. However, similar results are reported by FeGAN~\cite{fegan}. The reason is that, \algo can see the data five times per epoch as compared to the centralized approach which only sees it once. This boosts the diversity of samples seen by \algo thereby providing superior performance.
